Let's Play for Action: Recognizing Activities of Daily Living by Learning from Life Simulation Video Games

Recognizing Activities of Daily Living (ADL) is a vital process for intelligent assistive robots, but collecting large annotated datasets requires time-consuming temporal labeling and raises privacy concerns, e.g., if the data is collected in a real household. In this work, we explore the concept of constructing training examples for ADL recognition by playing life simulation video games and introduce the SIMS4ACTION dataset created with the popular commercial game THE SIMS 4. We build Sims4Action by specifically executing actions-of-interest in a "top-down" manner, while the gaming circumstances allow us to freely switch between environments, camera angles and subject appearances. While ADL recognition on gaming data is interesting from the theoretical perspective, the key challenge arises from transferring it to the real-world applications, such as smart-homes or assistive robotics. To meet this requirement, Sims4Action is accompanied with a GamingToReal benchmark, where the models are evaluated on real videos derived from an existing ADL dataset. We integrate two modern algorithms for video-based activity recognition in our framework, revealing the value of life simulation video games as an inexpensive and far less intrusive source of training data. However, our results also indicate that tasks involving a mixture of gaming and real data are challenging, opening a new research direction. We will make our dataset publicly available at https://github.com/aroitberg/sims4action.

==> sections/notes.tex <==
\clearpage
\input{IROS21/tables/results}

\begin{figure}
\begin{center}
\includesvg[width=0.5\textwidth]{figures/confm_test_split_s3d_no_pret} \\
\includesvg[width=0.5\textwidth]{figures/confm_test_split_s3d_no_pret_an}
\end{center}
   \caption{\david{I can easily provide these these confusion matrices in case you want to use them at some point.}}
\label{fig:rep_spaces}
\end{figure}

==> tables/results.tex <==
\begin{table}[t]
	\centering
	\scalebox{0.9}{
		
		\begin{tabular}{@{}ll|ccc|ccc@{}}
			
			\toprule
			\textbf{Model} &\multirow{2}{*}{\makecell{Weight \\ initialization}} & \multicolumn{3}{c|}{\textbf{SimsDataset Acc [$\%$] }} & \multicolumn{3}{c}{\textbf{Toyota ADL Acc [$\%$]}} \\
			&& Top 1 & Top 3 & Top 5 & Top 1 & Top 3 & Top 5 \\
			\midrule
			Random Baseline & None & 0.1 & 0.1 & 0.1 & 0.1 & - & - \\
			\midrule
			S3D & Random & 56.74 & 79.36 & 91.18 & - & - & - \\
			S3D & Kinetics400 & - & - & - & - & - & - \\
			I3D & Random & 67.00 & 87.81 & 94.29 & - & - & - \\
			I3D & Kinetics400 & - & - & - & - & - & -\\
			\midrule
			\bottomrule
		\end{tabular}
	}
	% 	\begin{tablenotes}
	% 	\item[a] Unbalanced training data
	% 	\end{tablenotes}
	\caption{Current available training results. The network is always trained on the SimsDataset and then either evaluated on the test set of the SimsDataset or the test set of the Toyota ADL dataset. The pretraining column refers to the network initialization before the SimsDataset training.\\
	Settings general: 64 frame sequences randomly selected within video sample chunks of 90 frames\\
	S3D: Batch size 16, img dim 128\\
	I3D: Batch size 10, img dim 224}
	\vspace{-0.3cm}
	\label{table:action_reco_results_current}
\end{table}

\begin{table}[t]
	\centering
	\scalebox{0.9}{
		
		\begin{tabular}{@{}ll|lccc@{}}
			
			\toprule
			\textbf{Model} & \textbf{Pre-Training} & \textbf{Type} & \multicolumn{3}{c}{\textbf{Toyota ADL Acc [$\%$]}} \\
			&&& Top 1 & Top 3 & Top 5 \\
			\midrule
		    S3D & Kinetics400 & cross subject & 32.19 & 62.20 & 73.77\\
		    S3D & Kinetics400 & cross view 1& 11.62 & 48.88 & 64.88\\
		    S3D & Kinetics400 & cross view 2 & 24.44 & 54.83 & 68.29\\
			\midrule
			S3D & Kinetics400 + Sims & cross subject & 38.57 & 68.14 & 77.28\\
		    S3D & Kinetics400 + Sims & cross view 1 & 39.32 & 59.03 & 72.44\\
		    S3D & Kinetics400 + Sims & cross view 2 & 46.90 & 70.13 & 80.75\\
			\midrule
		    I3D & Kinetics400 & cross subject & 29.41 & 48.50 & 64.92\\
		    I3D & Kinetics400 & cross view 1& 43.41 & 65.26 & 77.12\\
		    I3D & Kinetics400 & cross view 2 & 11.48 & 65.18 & 78.59\\
			\midrule
			I3D & Kinetics400 + Sims & cross subject & - & - & -\\
		    I3D & Kinetics400 + Sims & cross view 1 & - & - & -\\
		    I3D & Kinetics400 + Sims & cross view 2 & - & - & -\\
			\midrule
			\bottomrule
		\end{tabular}
	}
	% 	\begin{tablenotes}
	% 	\item[a] Unbalanced training data
	% 	\end{tablenotes}
	\caption{Results after a single epoch of transfer learning on the last layer only, other layers frozen.\\
	On S3D: Img dim 128, batch size 64, sequence length 30, learning rate 1e-4, wd 1e-4 with adam\\
	In I3D: Img dim 224, batch size 32, sequence length 30, learning rate 1e-4, wd 1e-4, adam}
	\vspace{-0.3cm}
	\label{table:action_reco_results_current}
\end{table}

==> tables/results_one_epoch_fine.tex <==
\begin{table}[t]
	\centering

		\scalebox{0.8}{
			\begin{tabular}{@{}llccc|ccc@{}}
			
			\toprule
			\textbf{Model} &\multirow{2}{*}{\makecell{Weight \\ initi.}} & \multicolumn{3}{c|}{\textbf{Normal Acc [$\%$] }} & \multicolumn{3}{c}{\textbf{Balanced Acc [$\%$]}} \\
			&& Top 1 & Top 3 &Top 5 & Top 1 & Top 3 &Top 5\\
			\midrule
			Random Baseline & None & 10.0 & 33.33 & 50.00 &10.0 & 33.33 & 50.00\\
			\midrule
			\textbf{Cross-subject} &  &  &  &  &  & \\
			Separable 3D Net & Kinetics &  &  &  &  &  &  & \\
			Separable 3D Net &  \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}}& &  &  &  &  &  & \\
			I3D  Net & Kinetics & 11.59 & 34.58 & 51.23 & 4.02 & 12.13 & 20.58\\
			I3D  Net & \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}} & 22.84 & 41.34 & 52.89 & 5.61 & 16.55 & 23.36\\
			 \midrule
			\textbf{Cross-view v1} &  &  &  &  &  & \\
			Separable 3D Net & Kinetics & &  &  &  &  &  & \\
			Separable 3D Net &  \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}}& &  &  &  &  &  & \\
			I3D  Net & Kinetics &  -& - & - & - & - & -\\
			I3D  Net & \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}} &  -& - & - & - & - & -\\
			 \midrule
			\textbf{Cross-view v2} &  &  &  &  &  & \\
			Separable 3D Net & Kinetics &  -& - & - & - & - & -\\
			Separable 3D Net &  \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}}& -& - & - & - & - & -\\
			I3D  Net & Kinetics &  -& - & - & - & - & -\\
			I3D  Net & \makecell[l]{Kinetics +\\
			 \textsc{Sims4Action}} &  -& - & - & - & - & -\\
			%C3D & None & - & - & - & - \\
			%C3D & Sports1M & - & - & - & - \\
			\midrule
			\bottomrule
		\end{tabular}
		}
	
	% 	\begin{tablenotes}
	% 	\item[a] Unbalanced training data
	% 	\end{tablenotes}
	\caption{One epoch finetuning }
	
	\label{table:finetune}
	
\end{table}


